Back in control -- An extensible middle-box on your phone

The closed design of mobile devices -- with the increased security and consistent user interfaces -- is in large part responsible for their becoming the dominant platform for accessing the Internet. These benefits, however, are not without a cost. Their operation of mobile devices and their apps is not easy to understand by either users or operators. We argue for recovering transparency and control on mobile devices through an extensible platform that can intercept and modify traffic before leaving the device or, on arrival, before it reaches the operating system. Conceptually, this is the same view of the traffic that a traditional middlebox would have at the far end of the first link in the network path. We call this platform ``middlebox zero'' or MBZ. By being on-board, MBZ also leverages local context as it processes the traffic and complements the network-wide view of standard middleboxes. We discuss the challenges of the MBZ approach, sketch a working design, and illustrate its potential with some concrete examples.

==> Makefile <==
###############################################################################
#
# File:         Makefile
# RCS:          $Id: Makefile,v 1.2 2011/01/31 20:29:00 fabianb Exp $
# Language:     Makefile
# Status:       Experimental (Do Not Distribute)
#
# (C} Copyright 2005, Northwestern University, all rights reserved.
#
###############################################################################


LATEX= latex
PDFLATEX=pdflatex
BIBTEX= bibtex
XDVI = xdvi
DVIPDF= dvipdfm -p letter
PS2PDF= ps2pdf
DVIPS= dvips -t letter -P pdf
RM = /bin/rm -f
CAT = cat
ISPELL = ispell
SORT = sort

MAINDOC = mbz
MAINPDF = ${MAINDOC}.pdf

DVIDOCS = ${MAINPDF:.pdf=.dvi} ${AUXPDF:.pdf=.dvi}
DVIDOCS = ${MAINPS:.ps=.dvi} ${AUXPS:.ps=.dvi}

all: ${MAINPDF} #${MAINPS} ${AUXPDF}


## enable bibtex but break if warning are raised
#%.pdf:  %.tex
#	${PDFLATEX} $*
#	if grep -s "^LaTeX Warning: Citation" $*.log ;  \
#	then \
#	        ${BIBTEX} $* ; \
#	        ${PDFLATEX} $* ; \
#	        ${PDFLATEX} $* ; \
#	fi ; \
#	while grep -s "Rerun to get cross-references right" $*.log ; \
#	do \
#	        ${PDFLATEX} $* ; \
#	done

## avoid stopping compile if bibtex raise warnings
%.pdf:  %.tex %.bib
	${PDFLATEX} $*
	${BIBTEX} $* ; \
    ${PDFLATEX} $* ; \
    ${PDFLATEX} $* ; \
	while grep -s "Rerun to get cross-references right" $*.log ; \
	do \
	        ${PDFLATEX} $* ; \
	done

%.ps: %.dvi
	${DVIPS} $*

%.dvi: %.tex
	${LATEX} $*
	if grep -s "^LaTeX Warning: Citation" $*.log ;  \
	then \
		${BIBTEX} $* ; \
		${LATEX} $* ; \
		${LATEX} $* ; \
	fi ; \
	while grep -s "Rerun to get cross-references right" $*.log ; \
	do \
		${LATEX} $* ; \
	done

%.bbl: %.bib
	${BIBTEX} $*

spell:
	${CAT} *.tex *.bib | ${ISPELL} -t -l | ${SORT} -u > spell.out

clean:	
	${RM} *.aux *.bbl *.dvi *.log *.blg *~ *.bak figs/*.bak

cleanAll: clean
	${RM} *.dvi *.ps *.pdf

distclean: cleanAll

